Painting 3D Nature in 2D: View Synthesis of Natural Scenes from a Single Semantic Mask

We introduce a novel approach that takes a single semantic mask as input to synthesize multi-view consistent color images of natural scenes, trained with a collection of single images from the Internet. Prior works on 3D-aware image synthesis either require multi-view supervision or learning category-level prior for specific classes of objects, which can hardly work for natural scenes. Our key idea to solve this challenging problem is to use a semantic field as the intermediate representation, which is easier to reconstruct from an input semantic mask and then translate to a radiance field with the assistance of off-the-shelf semantic image synthesis models. Experiments show that our method outperforms baseline methods and produces photorealistic, multi-view consistent videos of a variety of natural scenes.

==> exp/fid_2.tex <==
\begin{table}
\begin{subtable}[t]{0.4\textwidth}
\centering
\resizebox{0.2\textwidth}{!}{
\begin{tabular}{ccc}
\hline
% \vspace{-1em}
Methods & FID$\downarrow$ & KID$\downarrow$\\
% \hline
% SPADE~\cite{Park2019SemanticIS}      & 93.95 & 0.040 \\
\hline
(2) & 93.95 & 0.040 \\
(1) & 149.80 & 0.080\\
\hline
\end{tabular}

% \end{center}
% \vspace{-0.5em}
% \captionsetup{font={normalsize}} 
% \caption{\textbf{Quantitative comparisons on multi-view layout prediction.}}
% \vspace{-2em}
\label{table:fid_2}
}
\end{subtable}
\begin{subtable}[t]{0.4\textwidth}
\centering
\vspace{-1.5em}
\resizebox{0.2\textwidth}{!}{
\begin{tabular}{cccc}
\hline
% \vspace{-1em}
Methods & FID$\downarrow$ & NLL$\downarrow$ & VSC$\downarrow$\\
\hline
Ours & 93.95 & 0.040 & 0.040 \\
GVS & 149.80 & 0.080 & 0.040\\
\hline
\end{tabular}

% \end{center}
% \vspace{-0.5em}

% \captionsetup{font={normalsize}} 
% \caption{\textbf{Quantitative comparisons for layout generating.}}

\label{table:layout}
}
\end{subtable}
\end{table}


==> exp/layout.tex <==
% \begin{table}[bp]
% \centering
% \vspace{-1.5em}

% \begin{tabular}{cccc}
% \hline
% % \vspace{-1em}
% Methods & FID$\downarrow$ & NLL$\downarrow$ & VSC$\downarrow$\\
% \hline
% Ours & 93.95 & 0.040 & 0.040 \\
% GVS & 149.80 & 0.080 & 0.040\\
% \hline
% \end{tabular}

% % \end{center}
% \vspace{-0.5em}

% \captionsetup{font={normalsize}} 
% \caption{\textbf{Quantitative comparisons for layout generating.}}

% \label{table:layout}
% \end{table}


\begin{table}[hbp]
\vspace{-0.5em}
    \begin{subtable}[h]{0.23\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{ccc}
        \hline
        % \vspace{-1em}
        Methods & FID$\downarrow$ & KID$\downarrow$\\
        % \hline
        % SPADE~\cite{Park2019SemanticIS}      & 93.95 & 0.040 \\
        \hline
        SPADE+[32] & 149.80 & 0.080\\
        Ours & 109.85  & 0.050 \\
        \hline
        \end{tabular}
       }
       \caption{Table 1a.}
       \label{table:fid_2}

    \end{subtable}
    \begin{subtable}[h]{0.23\textwidth}
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{ccc}
        \hline
        % \vspace{-1em}
        Methods &  NLL$\downarrow$ & VSC$\downarrow$\\
        \hline
        Ours & 1.60 & 0.049 \\
        GVS &  3.33 & 0.089\\
        \hline
        \end{tabular}
        }
       \caption{Table 1b.}
        % \caption{\textbf{Layout generating.}}
        \label{table:layout}
    
     \end{subtable}
     % \caption{Max and min temps recorded in the first two weeks of July}
     % \label{tab:temps}
\vspace{-1em}

\end{table}

==> fig/vis_fuse_v1.tex <==
\begin{figure}
\begin{center}
    % \newcommand*\rot{\rotatebox{90}}
\setlength\tabcolsep{0.2em}
% \newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}
%  \newcommand{\myheight}{2cm}
\newcommand{\mywidth}{0.112 \textwidth}

\begin{tabular}{cc|cc}


\\

\multicolumn{2}{c}{Ours w/ semantic field}
&
\multicolumn{2}{c}{Ours w/o semantic field}
% \includegraphics[width=\mywidth]{fig/teaser/75224.png}
% & \includegraphics[width=\mywidth]{fig/teaser/76224.png}
% &\includegraphics[width=\mywidth]{fig/teaser/77224.png}
% &\includegraphics[width=\mywidth]{fig/teaser/78224.png}\\
\end{tabular}
\end{center}
\captionsetup{font={normalsize}} 
\caption{\textbf{The effect of involving semantic field.} The first two columns and the last two columns are adjacent frames. Without the involvement of a semantic field, images are generated with artifacts. } 
\label{fig:vis_fuse_v1}
\end{figure}

    

==> fig/zero.tex <==
\begin{figure}[bp]
\setlength\tabcolsep{0.1em}

\newcommand{\mywidth}{0.11 \textwidth}
\centering
\vspace{-1.2em}

\begin{tabular}{ccc}

\includegraphics[width=\mywidth]{fig/zero/001.png}
&\includegraphics[width=\mywidth]{fig/zero/075.png}
& \includegraphics[width=\mywidth]{fig/zero/329.png} \\
 \footnotesize Input image
&\footnotesize Novel view
& \footnotesize Warped back


\end{tabular}

\vspace{-1em}
\captionsetup{font={normalsize}} 
\caption{\textbf{Results of [32].}}
\vspace{-2em}

\label{fig:zero}
\end{figure}

==> sec_1_intro_v2.tex <==
% TODO: 改名字和semantic view synthsis不一样-> 说3D scene generation？
% 去掉infinite nature直接引出我们的方法确实还行

\section{Introduction}
\label{sec:intro}

% 1. 我们的setting是用利用single-view dataset的先验去optimizie 一个neural field
% 2. 然而这样的事情是非常困难的
% 3. 从单张semantic mask neural field for 3D natural scene这件事情是没有被探索过的。一些3D GAN的工作只能在object-centric数据集上work。
% 4. semantic mask没有appearance信息，难以让neural field学到appearance信息，更别说geometry了。 
% 5. 虽然我们可以先将semantic mask转换成RGB图片。但是如何从单目图片生成一个3D natural scene仍然是一个非常困难的事情。
% 6. 先前有工作使用posed video去学习获得prior， 但是posed natural videos的获得非常困难。如何让这些工作在single view dataset上训练仍然没被探索。
% 7. 讲我们的方法
 
%然而这些算法只能生成2D的图片，很少有工作关注semantic view synthesis这样的任务。semantic view synthesis是从单张2D semantic map出3D representation并且生成novel view的任务。semantic view synthesis这个任务可以帮助人们通过semantic map快速生成自己想要的3D内容，为人们创作三维内容提供了友好的工具。
%一些工作GVS(Generative View Synthesis: From Single-view Semantics to Novel-view Images)，SVS（Semantic View Synthesis）可以从2D semantic map生成free viewpoint video，并且取得了promising的效果。这些工作利用posed video训练（given posed videos for training），通过input semantic map推理出MPI，在target views上渲染，通过target views的GT监督网络训练。然而使用posed video限制了他们view synthesis的效果和style多样性。因为获得非常多的video不是一件轻松的事情，我们很难收集充足的posed video训练这个模型。并且预测精准的camera pose更加是一件困难的事情，如果camera不准那么将会产生错误的监督信号导致效果下降。（https://infinite-nature-zero.github.io/static/pdfs/InfiniteNatureZero.pdf）如何使用自然Internet数据集训练得到可以做semantic view synthesis的model仍然还是一件没有被人探索的事情。（it would be interesting if we can achieve semantic view synthesis by training the model on 在室外自然数据集上）

% 1. 我们的setting是从a single semantic mask恢复3D renderable representation of natural scene for view synthesis. 有很多应用.
% 2. 介绍我们想从train a neural field of natural scene that admits the structure indication of the semantic mask.
% 3. 然而这样的事情是非常困难的.
% 4. semantic mask没有appearance信息，难以让neural field学到appearance信息。 
% 5. 一个方法是训练一个2D generator, 将semantic mask转换成RGB图片。但是如何从单目图片生成一个3D natural scene仍然是一个非常困难的事情。只有SinNeRF探索了object-level的single-view neural field reconstruction.
% 6. 讲我们的方法
%
3D content creation has many important applications in AR/VR, data augmentation, and robotics.
%
The continuous effort of exploring advanced deep generative models has revolutionized content creation -- synthesizing photo-realistic images is now made possible.
%
Some methods~\cite{park2019semantic,sushko2020you,wang2018high,isola2017image} condition generative models on semantic masks, thereby enabling them to edit generated images by revising semantic masks, 
%
which greatly facilitates humans' creation of image contents.
%
Albeit the stunning results, most semantics-driven generation methods produce 2D images, without considering the underlying 3D structure of the world.
%
\ctr{However, in the future, applications like navigation, gaming, and virtual reality, will intensively rely on 3D content. The huge demand for 3D content brings an unprecedented demand for generating 3D representations by machines.}
%

\zsz{In this work, we aim to extend the content generation in the 3D world, with a particular focus on a novel task of semantics-guided
scene generation.} \ctr{Witnessing the recent success in the neural field as a 3D representation in many downstream tasks, this task aims to train a neural field for a natural scene guided by a single semantic mask. Similar to 2D image generation, our scene generation admits the structure indication of the single semantic mask and aims to produce view-consistent and photo-realistic results in 3D. 
However, training a neural field using a single semantic mask is extremely hard, considering the fact that training a neural field for a natural scene from a single image remains unexplored, let alone from a single semantic mask. It is particularly challenging for a neural field to learn the texture of the 3D world, as the semantic mask does not contain appearance information.}


A naive solution is to directly combine 2D image-to-image translation techniques with 3D representation, which first utilizes image to image translation technique to convert the semantic mask to an RGB image and then uses the RGB image to recover a neural field. However, optimizing a neural field on a single natural image is still challenging, as shown in~\cite{xu2022sinnerf,yu2021pixelnerf}.
% In this work, we focus on the task of semantics-guided scene generation, which aims to create free-viewpoint rendering of 3D scenes from a single-view semantic mask.
% To overcome this problem, we aim to produce 3D scene representations from single-view semantic maps and create free-viewpoint rendering of 3D scenes.
\zsz{Recent semantic view synthesis methods \tocite{svs, gvs} train their models on datasets \tocite{training datasets of svs} consisting of posed videos.
...}
%The continuous effort of exploring advanced deep generative models has revolutionized content creation -- synthesizing photorealistic images is now made possible.
%%
%Often, the generative model synthesizes content with conditions on certain input data.
%%
%A widely-used input modality is semantic masks, which can be drawn by humans and used for photo-realistic image synthesis and editing, greatly facilitating humans' creation of new content.
%%
%Albeit the stunning results, existing semantic-driven content creation is mostly for 2D images. In this work, we aim to extend the capability of semantic content synthesis to the 3D world -- allowing users to use 2D semantic masks to produce content in 3D. 
%%
%Specifically, we focus on the task of semantic view synthesis, which takes input from a 2D semantic mask and produces a 3D representation.
%%
%Based on the 3D representation, novel view synthesis can be performed so that users can view a scene in 3D, which provide a valuable tool for 3D content creation, especially in the context of AR/VR.

% 1. 训练generative models需要大量的数据。
% 2. SVS在posed videos上训练。
% 3. SVS具体怎么做的。
% 4. However, a large number of videos with calibrated camera poses are hard to obtain in real life, which limits the diversity of training data.
% 5. Moreover, it is also easy to introduce errors from inaccurate camera poses, thus restricting the performance of learned generative models.


%
%Moreover, it is also easy to introduce errors from inaccurate camera poses, thus restricting the performance of learned generative models.

%Obviously, producing photorealistic results using neural networks stands on the foundation of large-scale and diverse training data.
%%
%Existing methods \tocite produce multi-plane images (MPI) from the semantic masks and render the image at a novel viewpoint, which is supervised by the ground truth images from posed videos.
%%
%However, a large number of videos with calibrated camera poses are hard to obtain in real life; it is also easy to introduce errors from inaccurate camera poses, thus restricting the quality of synthesized images.

% Alternatively, many tasks facing restrictions from the dataset have been working on using millions of images from the Internet. Tasks like panorama generation \tocite, image extrapolation \tocite, and image editing \tocite have benefited from versatile large-scale Internet images. However, no previous work of semantic view synthesis has used Internet images. 

% 1. 一个解决方法是利用single-view image collections来学习semantic view synthesis models。
% 2. Li et al. have utilized such data to train a neural network which performs novel view synthesis given a single view image.
% 3. Specifically, Li怎么做novel view synthesis的 -> Li怎么训练neural network的
% 4. It is easy to extend such an approach to semantic view synthesis through a two-stage scheme: first converting the semantic map to an RGB image and then performing the novel view synthesis.
% 5. However, Li在image space生成图片，and big 2D CNNs难以生成view-consistent images, as discussed in \tocite.

% TODO: 要不要改成讨论AdaMPI，感觉这篇论文比Li的论文更强。不会有view inconsistent的问题。
% TODO: AdaMPI的做法是拿Li的模型训练SVS。感觉讨论AdaMPI可能有点多余。但不讨论，这里讨论Li的方法，又不太能引出我们的方法。这一段没有抛出一个技术挑战
% TODO: 这里可以讨论从single-view image恢复3D representation不好的问题，作为我们方法要解决的技术挑战
%老师说去掉这段放在related work

%Recently, \cite{Li2022InfiniteNatureZeroLP} have utilized Internet images to perform novel view synthesis from single-view images by warping source images to random target views and wrapping back to train the RGB inpainting network to produce complete and coherent novel view images.
%%
%It is easy to extend such an approach to semantic view synthesis by first converting the semantic masks to RGB images and then performing the novel view synthesis.
%%
%However, this approach is not view-consistent due to the lack of shared 3D representations during the wrapping process.
%%
%As a unique demand of 3D synthesis tasks, the view consistency of the output is particularly important besides photo-realism. 

% 这段话不用说。因为不是我们的贡献。大家都知道view inconsistency可以被3D representations缓解
% 不要描述baseline，不然别人会觉得我们方法只是多加了semantic field
% We argue that view inconsistency can be alleviated by learning 3D representations, such as MPI and neural radiance field (NeRF), which are a promising 3D representation that has demonstrated vast possibilities in 3D content reconstruction and synthesis. We can use NeRF to fuse images wrapped to different views and use it for novel view synthesis by rendering at arbitrary viewpoints. However, as the input images for optimizing NeRF are not view-consistent, severe blurring and artifacts exist in the output results, as our experiment shows. 

% 讲通过neural field利用spade的advance，得到高质量的3D scene
% 另一个关键是semantic neural field，所以才能很好地利用spade的advance
% 两个contribution：1. 通过neural field利用2D generator实现semantic view synthesis. 2. 通过semantic neural field提升渲染质量

% 1. In this paper, we propose a novel framework for generating renderable 3D representations from single-view semantic maps.
% 2. Our key idea is exploiting neural fields to obtain high-quality 3D representations from the advanced 2D semantics-driven generators \tocite{spade, and so on}, which are well trained on single-view image collections.
% 3. Specifically, given a semantic map, 我们先得到semantic neural field，从而得到multi-view semantic maps.
% 4. 然后用spade得到multi-view images，用于训练一个renderable 3D representations，用于view synthesis.

We propose a novel framework for generating renderable 3D representations from a single-view semantic mask.
%
Our key idea is exploiting neural fields to obtain high-quality 3D representations from the advanced 2D semantics-driven generators \tocite{spade, and so on}, which are well-trained on single-view image collections.
%
Specifically, we innovatively reconstruct a semantic neural field from the input semantic mask, which is used to produce multi-view semantic masks.
%
Then, the 2D semantic image synthesis model SPADE is leveraged to generate multi-view images from semantic masks.
%
Considering generated images of SPADE could be view-inconsistent\zsz{ at the semantic level}, we further optimize a renderable 3D representation from multi-view images for novel view synthesis.

% 讲先得到semantic neural field的好处
% 1. 和先得到image，再得到3D representation的方法相比，我们方法有两个优势。
% 2. 一是单张semantic map得到semantic neural field比单张图得到nerf简单。
% 3. 二是得到multi-view semantic maps以后，可以充分利用spade的generation capacity。


Our approach has two advantages.
%
First, we observe that semantics has lower complexity than scene appearance, leading to the fact that reconstructing semantic neural fields from a single-view semantic map is much easier than reconstructing renderable representations from RGB images.
%
Second, based on the multi-view semantic masks, we can fully utilize the powerful generation capacity of SPADE at multiple viewpoints.
%
\zsz{Finally, compared to  directly combining the 2D image-to-image translation techniques with 3D representation, our method fully utilize the semantic information, thus leading to more photo-realistic results}
%
% In contrast, SVS \tocite{svs} only applies SPADE on a single viewpoint.

%We hereby offer a nascent approach trained only on the Internet natural images to perform semantic view synthesis that substantially differs from the existing method.
%%
%We make a key observation that semantic label maps, as a low-level manifold, are easier to be inpainted or fused.
%%
%Based on the observation, instead of using inconsistent multi-view RGB images generated by semantic label maps to learn the 3D representation, we propose a novel approach that directly uses a single semantic mask to synthesize a 3D representation, namely semantic field, and use the semantic field to guide the learning of color field and perform novel view synthesis.
%%
%By disentangling semantic information and RGB information, our two-stage approach simplifies the task and better exploits the semantic information to guide novel view synthesis.

% 不要说我们是the first
% To the best of our knowledge, we are also the first to use a single semantic mask to synthesize a complete neural field and generate high-quality videos viewed from a wide range of viewpoints.
%
We have performed extensive experiments with the recent several strong baselines to verify the effectiveness of our approach.
%
We show that our method outperforms existing methods both qualitatively and quantitatively with state-of-the-art (SOTA) performance.

In summary, this work has the following contributions:

\begin{itemize}[leftmargin=*]
\vspace{-\topsep}
\item We are the first to introduce a novel framework which can perform semantic view synthesis with solely unstructured monocular 2D natural images from the Internet for training. Our framework removes the dataset's constraint and frees the need to obtain expensive and well-calibrated multi-view data.

%We introduce a novel framework, which exploits a single semantic label map to synthesize free-viewpoint videos and is able to train on the readily-available unstructured 2D image datasets
%task
%framework+observation - semantic field+state-of-the-art
\item We make a key observation that semantic masks are easy to be inpainted in 2D and fused in 3D. We thus propose a novel two-stage approach that exploits a single semantic mask to first form a 3D semantic field and then synthesize colored 3D content. 
\item \ky{Our method surpasses existing methods and constitute as the state-of-the-art on semantic view synthesis of nature scenes. As such, we can generate photo-realistic and geometry-consistent novel-view images from a single mask. }
% Our method outperforms the existing method with state-of-the-art results on semantic view synthesis of nature scenes. With only a single semantic mask, 3D content of high-quality, photo-realistic, and view-consistent novel view synthesis is realized. 
\end{itemize}




 


%Recent years have witnessed great advances of image synthesis using deep generative models. Photo-realistic images can be synthesised 


==> sec_2_related.tex <==

\section{Related Works}
\label{sec:formatting}

%-------------------------------------------------------------------------
\subsection{Semantic View Synthesis}
Semantic view synthesis is a task that takes input from a 2D semantic mask and produce a 3D representation. To generate 3D representations from a single semantic map and render novel views, SVS~\cite{Huang2020SemanticVS} and GVS~\cite{Habtegebrial2020GenerativeVS} combine 
multi-plane images (MPI)~\cite{Zhou2018StereoML} and image-to-image translation techniques~\cite{Park2019SemanticIS}, achieving promising results. However, they need posed videos to train their models. Because it is challenging to obtain a large collections of posed videos in the wild, their methods are not easy to be applied in the Internet natural datasets.
 

\subsection{Single-view View Synthesis}
Recently, single-image view synthesis~\cite{kopf2020one, hu2021worldsheet,han2022single, Wiles2020SynSinEV, Shih20203DPU,Li2022InfiniteNatureZeroLP,Liu2021InfiniteNP,Niklaus20193DKB,Tulsiani2018Layerstructured3S,Park2022BridgingIA,Rockwell2021PixelSynthGA,Rombach2021GeometryFreeVS,Ren2022LookOT} 
has received wide attention. Some works use explicit 3D representations, such as 
layered depth image (LDI)~\cite{Hedman2018Instant3P, shade1998layered} and multiplane image (MPI)~\cite{Zhou2018StereoML}, 
can render novel views from a single image, by capturing visible contents and inferring occluded contents.
Another line of researchs predict neural radiance field~\cite{mildenhall2021nerf} from a single image. PixelNeRF~\cite{yu2021pixelnerf} extracts image feature by using
2D CNN and construct aligned feature field to render novel view. 
MINE~\cite{li2021mine} combine MPI and NeRF representation and learn a continuous 3D field. 
A common scheme for training these representations is to supervise a network that can predict a 3D scene representation by using multi-view images or videos and assuming relative camera poses between the different images are known. 
However, there aren't many large-scale multiview datasets available, so it's challenging to apply these techniques to the natural Internet datasets.

To train the models on the in-the-wild dataset, 
\cite{kopf2020one} and \cite{Shih20203DPU} use monocular depth estimation network to construct LDI representation and leverage inpainting network to synthesize occluded content, which can be trained on the in-the-wild dataset. 
Another works propose a warp-back training strategy~\cite{han2022single} or cyclic virtual camera trajectory~\cite{Li2022InfiniteNatureZeroLP} for self-supervised training strategy to train inpainting network in the wild.
 SinNeRF~\cite{xu2022sinnerf} directly train the NeRF given a single rgbd image input without any prior from multi-view datasets. Aforementioned works focus on render novel views from a single rgb image, but our work concentrate on synthesize novel view from a single semantic map. 


\subsection{Neural Radiance Field}
Neural Radiance Field~\cite{mildenhall2021nerf} and its extended works 
have significantly promoted the state-of-the-art in novel view synthesis~\cite{zhang2020nerf++, barron2022mip, barron2021mip, peng2021neural, chen2021mvsnerf,niemeyer2022regnerf}, 3D reconstruction~\cite{oechsle2021unisurf,zhang2022nerfusion,ehret2022nerf}, and 3D generative modeling~\cite{schwarz2020graf, schwarz2022voxgraf,niemeyer2021giraffe,chan2021pi}. 
Most above works focus on rendering realistic novel view images or reconstructing accurate 3D geometry, but how to generate NeRF from a single semantic map still remains to be explored. 
Semantic-NeRF~\cite{zhi2021place} and its following works~\cite{fu2022panoptic, kundu2022panoptic,tschernezki2022neural} have shown NeRF is a powerful 3D fusion tools. 
However, they can not construct 3D semantic field from only a single semantic map and do not explore how to generate appearance and geometry from semantic field. 
Another line of works~\cite{chen2022sem2nerf,sun2022fenerf,sun2022ide} extend 3D generative modeling to edit 3D appearance and geometry via a semantic map, but they focus on simple object (e.g. faces) from carefully prepared datasets with known camera distribution and fail to generate complex scene like landscapes from the in-the-wild dataset. 
A closely related work Gancraft~\cite{hao2021gancraft} and its extended work~\cite{jeong20223d} use image-to-image translation techniques~\cite{park2019gaugan,park2019semantic,sushko2020you,wang2018high} to synthesize pseudo ground truths and discriminator to make generative free-viewpoint videos more realistic from 3D semantic labels. Nevertheless, they need 3D semantic labels to render consistent 2D semantic maps and fail when only takes a single semantic map as input.  


\subsection{Image-to-image Translations}
Image-to-image translations~\cite{park2019gaugan,park2019semantic,sushko2020you,wang2018high} has made tremendous development and can synthesize realistic landscape images. 
Pix2Pix~\cite{isola2017image} firstly leverages conditional GAN~\cite{mirza2014conditional} to improve performance of semantic image synthesis. SPADE~\cite{park2019semantic} proposes spatial-varying normalization layer and significantly improves the image synthesis performance. 
OASIS~\cite{sushko2020you} propose a novel discriminator to get rid of VGG loss~\cite{johnson2016perceptual}. However, these works can only synthesize 2D images and are not able to generate images of different views. 


==> sec_3_method.tex <==
\section{Method}
% 这一段的写作思路
% 1. Our goal is performing view synthesis of natural scenes from a single semantic map.
% 2. To this end, given a semantic map, we recover a neural 3D scene reprensetation for novel view synthesis, whose appearance is controlled by style codes.
% 3. In this section, we first introduce how to reconstruct a semantic neural field from a single semanitc map (Section~\ref{ssnerf}).
% 4. Then, Section~\ref{ssnerf} discuss how to learn style-controlled neural renderer from the semantic neural field.
% 5. Finally, we describe the training produce in Section~\ref{sgt}.
% TODO: 根据写作思路改一下这一段话
Our goal is overfiting a neural field and rendering novel views from a semanitc map according to the user-controlled camera trajectories and 
style code $z$.
%
Fig x gives an overview of our novel pipeline. We first introduce our novel appoarch which can synthesize a semantic neural field from a single semanitc map in section \ref{ssnerf}. 
%
Then, we use our semantic neural field to render consistent semantic label maps and extract the surface. 
%
In section \ref{sgr}, we describe our surface-guided rendering and a triplane-based color field generator. 
%
To train our color field, we introduce our semantic-guided training procedure in section \ref{sgt}.

\subsection{Learning semantic neural fields}\label{ssnerf}
%
% TODO: 这段话可以去掉。和上一段话重复了。如果想介绍motivation，就在介绍完方法以后写motivation
Directly training a 3D representation which can render freeviewpoint videos on a sinlge semantic map is too challenging.
%
To tackle this challenging problem, our key idea is firstly construct a semantic neural field from a single semantic maps and then train a color field guided by obtained semantic neural field. 
%
To this end, we propose our novel appoarch which can lift a single semantic map to a 3D semantic field.
This module combines 3D rendering, semantic inpainting networks and semantic field in a novel way.

% TODO: 写一段overview，描述一下怎么learn semantic neural fields。如果不写这个，读者很容易不知道在做啥。写作思路:
% 1. Figure X presents the overview of training semantic neural fields from the semantic map.
% 2. Given a semantic map, our approach first generates multiple semantic maps at novel views.
% 3. 然后...
% 4. 最后...

\paragraph{Generating multi-view semantic maps.}\label{sw}
% TODO: 补上写作思路
% 0. 一句话简单讲一下overview
% 1. 首先得到RGB image
% 2. 然后得到monocular depth
% 3. 然后根据monocular depth得到triangular mesh
% 4. 然后根据triangular mesh做warping
% 5. 最后用mesh renderer得到semantic maps at novel views
%
% TODO：corresponding monocular depth map哪来的。这里突然出现一个输入或新名词会让人觉得奇怪
% TODO：可以改成 Our appoarch warps the given semantic map to novel views through the depth-based warping technique. 如果讲技术，就不会让人奇怪, 因为大家一般听说过这个技术。注意，不要突然出现一个输入或新名词。
Our appoarch warps the given semantic label map to novel views according to the corresponding monocular depth map. 
%
% TODO: 根据写作思路改一下后面几句话
To obtain the corresponding depth map, we firstly apply spade to convert the given semantic map to the corresponding RGB image and then use monocular depth estimation networks~\cite{ranftl2020towards} to predict the depth map from the generated RGB image. 
%
% TODO: 3D triangular mesh哪里来的。不要突然出现一个输入或新名词。
After obtaining depth map, we lift the semantic map into a 3D triangular mesh by treating each pixel as vertices and connecting them with their neighbors. 
% TODO: method有三个元素组成：输入、要解决的问题、技术。“输入”和“要解决的问题”要介绍清楚，不能“突然出现”。如果用别人的技术，需要cite。如果是自己的技术，要讲清楚。
% TODO: 输入、problem，这两个需要介绍怎么出来的
%
% TODO: suprious edges哪里来的。不要突然出现一个输入或新名词。
To get rid of spurious edges, we remove the edges at depth discontinuities according to the gradient of the depth map.
%
% TODO: mesh renderer是一个技术，需要引用一下之前的方法。
% TODO: we warp the semantic label map to the novel views based on a mesh renderer following \tocite.
Finally, we warp the semantic label map to the novel views using a mesh renderer.

\paragraph{Semantic Inpainting}\label{sr}
% TODO: 这段写作思路不太清楚。写之前要先列一下写作思路，确定思路是清楚的。
%
After directly warping the given semantic map to novel views, there exist many invisible areas at novel views.
%
% TODO: 为了infer the invisible contents at novel views, 我们train a semantic inpainting network做什么。什么是semantic inpainting network。什么是Internet dataset, 有这样的说法吗
% TODO: To overcome this problem, we train an inpainting network to fill in contents of semantic maps at these regions. The inpainting network is trained on the LHQ dataset~\cite{skorokhodov2021aligning}.
To infer the invisible contents at novel views, we train a semantic inpainting network on the Internet Dataset, LHQ~\cite{skorokhodov2021aligning}.
%
% TODO: 接下来几句话的思路不清楚，建议改成。建议写一遍思路，再写成最终的英语句子，不用直接上手写最终的句子
% 1. We adopt a warp-back training strategy similar to~\cite{han2022single}.
% 2. Specifically, given the LHQ dataset, 我们用DeepLab to produce segmentation maps and depth maps for each image.
% 3. Then, we use the depth map to warp the semantic map to a random target view $S_0'$, and then warp it back to the source view, which gives a semantic map with holes.
% 4. Finally, we input $\hat{S_0}$ to the inpainting network to predicted the complete semantic map.
% 5. The predicted semantic map is compared with the original semantic map to optimize the inpainting network.
% 6. After training, we warp the given semantic label map to each novel view and apply the inpainting network to fill in their invisible areas, thus obtaining multiview semantic label maps. 
In order to prepare the LHQ dataset to generate training data of our semantic inpainting networks, we first use pretrained DeepLab-v2~\cite{chen2017deeplab} to produce pseudo segmentation annotations and then use monocular depth estimation~\cite{ranftl2020towards} to predict the depth maps.
%
We adopt a warp-back training strategy similar to~\cite{han2022single}. 
%
In details, we warp the source semantic label map $S_0$ to a random target view $S_0'$, and then warp it back to the source view to synthesize the semantic label map $\hat{S_0}$ with naturalistic invisible areas. 
%
% TODO: "fill in invisible areas with the ground truth"这句话写的有问题
Lastly, we input $\hat{S_0}$ to the semantic inpainting networks and train the networks to fill in invisible areas with the ground truth $S_0$. 
%
After training, we warp the given semantic label map to each novel view and apply the inpainting network to fill in their invisible areas, thus obtaining multiview semantic label maps. 

% After directly warping the given semantic map to novel views, there exist many invisible areas at novel views.
% %
% To infer the invisible contents at novel views, we train a semantic refinement network on the Internet Dataset, LHQ.
% %
% In order to prepare the LHQ dataset to generate training data of our semantic refinement networks, we firstly use pretrained DeepLab-v2 to produce pseudo segmentation annotations and then use monocular depth estimation to predict the depth maps. We adopt a warp-back training strategy similar to Adampi.
% %
% In details, we warp the source semantic label map S0 to a random target view S0', and then warp it back to the source view to synthesize the semantic label map $\hat{S0}$ with naturalistic invisible areas.
% %
% Lastly, we input $\hat{0}$ to the semantic refinement networks and train the networks to fill in invisible areas. After training, we warp the given semantic label map to each novel view and apply semantic refinement network to fill in their invisible areas, thus obtaining multiview semantic label maps.

\paragraph{Semantic Field Fusion}
%
% TODO: "can not" -> "cannot". "section \ref{sr}" -> "Section~\ref{sr}". 有这个问题的都要改掉
Although we obtain multi-view semantic label maps in section \ref{sr}, we can not directly use these semantic label maps to guide the training of view synthesis. 
%
% TODO: "multiview" -> "multi-view"
Because these multi-view semantic label maps are not view consistent, directly using these semantic label maps will cause artifacts. 
%
To tackle this problem, we introduce a semantic neural field to fuse multi-view semantic label maps and then render view consistent semantic label maps.
%
% TODO: 接下来写作的思路不清楚，不用先说问题，再说做法。如果不先把semantic neural field定义清楚，别人不知道我们在优化什么。直接讲怎么做的：
% 1. Semantic neural field的定义
% 2. 训练Semantic neural field的loss
% TODO: "how to overfit a semantic field on a single 2D semantic map"这句话有点问题, 因为我们已经有multi-view semantic maps了。
However, how to overfit a semantic field on a single 2D semantic map is a really challenging problem. 
%
% TODO: "can not" -> "cannot". 有这个问题的都要改掉
Neural field needs multi-view RGB images or depth maps to learning 3D geometry, but multi-view semantic label maps can not provide sufficient 3D supervision.
%
Inspired by previous methods~\cite{wang2022neuris,yu2022monosdf}, we use monocular depth maps to supervise the neural field.
%
In details, we firstly use depth map at the reference view obtained by \ref{sw} to supervise neural field.
%
To better leverage the geometry information of this depth map, we also warp the depth map to novel views using the mesh renderer to train neural field.

%
However, the depth values at invisible areas at the novel view is still unknown.
%
% TODO: 这里不用再讲之前的方法。直接说：To handle this problem, we adopt a simple but effective way to supervised the learned geometry at these areas.
Instead of using depth inpainting networks as in \cite{Shih20203DPU,Li2022InfiniteNatureZeroLP,Liu2021InfiniteNP,han2022single} to fill in these areas, we adopt a simple but effective way to synthesize resonable geometry information of these areas.
%
% TODO: "unkown" -> unknown, 其他地方也要改一下
We consider the monocular depth map as a relative cue and constrain the rendered depth at these unkown areas to match this relative cue.
%
% TODO: "firstly" -> first, 其他地方也要改一下
We firstly convert the semantic map at novel views to RGB images via SPADE and then use monocular depth estimation networks~\cite{ranftl2020towards} to predict depth maps.
%
We enforce rendered depth map $\hat{D_i}$ at novel view $i$ consistent with the predicted monocular depth map $D_i$ at novel views $i$ by ranking loss~\cite{chen2016single, xian2020structure}, as shown in equation~\ref{rank}.
%
To constrain the 3D geometry and obtain a well-defined surface, we adopt SDF-based volume rendering. 
\begin{small}
\begin{equation}\label{rank}
\begin{aligned}
loss(p_0, p_1)= \begin{cases}\log \left(1+\exp \left(-\ell\left(p_0-p_1\right)\right)\right), & \ell \neq 0 \\ \left(p_0-p_1\right)^2, & \ell=0\end{cases}
\end{aligned}
\end{equation}
\end{small}
where $j$, $k$  denote the locations of the randomly sampled pixels at novel view $i$. $p_0=\hat{D_{ij}}$ and $p_1=\hat{D_{ik}}$ is the rendered depth values at location $j$ and $k$.
$\ell$ is induced by the predicted monocular depth $D_i$ and a tolerance threshold $\tau$. 
$p_0^*=D_{ij}$, $p_1^*=D_{ik}$ are the the predicted monocular depth values at location $j$ and $k$:
\begin{small}
\begin{equation}\label{ol}
\ell= \begin{cases}+1, & p_0^* - p_1^*>=\tau \\ -1, & p_0^* - p_1^*<=\tau \\ 0, & \text { otherwise }\end{cases}
\end{equation}
\end{small}

% TODO: 这里讨论learning semantic neural fields的motivation和好处

\subsection{View Synthesis Based on Semantic Field}

\subsubsection{Surface-guided Rendering}\label{sgr}
% TODO: 先写一遍思路，再写成最终的英语句子，不用直接上手写最终的句子
%
We use the geometry recovered by semantic neural field to guide image synthsis.
%
Because volume rendering lacks surface constraint and is prone to be view-inconsistent without multi-view supervision, we adopt surface guided rendering instead of volume rendering to ensuring multi-view consistency.
%
We extract mesh from neural SDF field and use the mesh to guided ray sampling. 
%
Similar to~\cite{lin2021efficient},  we only query one point on the surface for each pixel. We follow EG3D~\cite{chan2022efficient} and use a tri-plane representation to represent our color field.
%
The points on the surface are projected to each feature plane to aggregate the feature F. The concatenated feature vector F is then mapped to the RGB color c by MLPs.
%
Additional advantage of adopting surface-guided rendering is that we can minimize the computational burden of producing high-resolution images, achieving efficient training and fast rendering. 

\subsubsection{Semantics-guided Training}\label{sgt}
% TODO: 先写一遍思路，再写成最终的英语句子，不用直接上手写最终的句子
%
We train our color field guided by semantic neural field with reconstruction and adversarial losses.
%
To make the training more stable and faster, we generate pseudo-ground images to supervise our color field.
%
The pseudo ground-truth images are synthetized by SPADE conditioning on the semantic label map rendered by our semantic neural field.
%
With the reconstruction loss, the error between the rendered images and the corresponding pseudo-ground image is reduced.
%
Additionally, we use the adversarial loss to make the rendered images more photorealistic and ensure our rendered images condition on the semantic labal maps.
%
We adopt OASIS discrimintor, which can provide stronger supervision to generator, to supervise our color field.
%
The advantage of our semantic guided training procedure is that we can ensure the semantic consistency between different views.
%
Therefore, pseudo ground-truths generated by spade only differ in local texture, which is much easier for the neural field to fuse.

\subsubsection{Style Controlling}
% TODO: 先写一遍思路，再写成最终的英语句子，不用直接上手写最终的句子
To make the style of our rendered video controllable, our designed triplane generator and SPADE are conditioned on the style code z.
%
During the training,  We random sample style code z from Gaussian distribution N.



==> sec_3_method_v2.tex <==
\section{Method}
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth]{fig/method/method1.pdf}
\vspace{-1em}
\caption{\textbf{Pipeline.} }
\label{fig:pipeline}
\end{figure*}
% TODO: setting里要突出只在单目数据集上训练
% 这一段的写作思路
% 1. Our goal is performing view synthesis of natural scenes from a single semantic map.
% 2. To this end, given a semantic map, we recover a neural 3D scene reprensetation for novel view synthesis, whose appearance is controlled by style codes.
% 3. In this section, we first introduce how to reconstruct a semantic neural field from a single semanitc map (Section~\ref{ssnerf}).
% 4. Then, Section~\ref{ssnerf} discuss how to learn style-controlled neural renderer from the semantic neural field.
% 5. Finally, we describe the training produce in Section~\ref{sgt}.
Our goal is to perform photo-realistic view synthesis of natural scenes given a single semantic mask and only utilize single-view natural image collections to train our models.
%
To this end, we leverage a pre-trained 2D semantics-driven generator to learn a neural scene representation for view synthesis.
%
In this section, we first introduce how to reconstruct a semantic neural field from a single semantic mask (Section~\ref{ssnerf}).
%
Then, Section~\ref{sgr} discusses how to learn a neural renderer based on the semantic neural field and the pre-trained 2D generator.
%
Finally, we describe the training procedure in Section~\ref{sgt}.

% Fig x gives an overview of our pipeline. We first introduce ourf appoarch which can synthesize a semantic neural field from a single semanitc map in section \ref{ssnerf}. 
%
% Then, we use our semantic neural field to render consistent semantic label maps and extract the surface. 
%
% In section \ref{sgr}, we describe our surface-guided rendering and a triplane-based color field generator. 
%
% To train our color field, we introduce our semantic-guided training procedure in section \ref{sgt}.

\subsection{Learning Semantic Fields}\label{ssnerf}

Figure\tocite illustrates the overview of our approach of learning a 3D semantic field from a semantic mask $S_0$.
%
%
Given a semantic mask, we first warp the given semantic mask to novel views. 
%
Then, an inpainting network is utilized to fill in the disocclusion areas of the warped semantic mask at each novel view.
%
After obtaining an inpainted semantic mask\yl{After obtaining multiple inpainted semantic masks of different viewpoints}, we recover a semantic field that can fuse this multi-view semantic information.

\paragraph{Warping Semantic Mask.}\label{sw}
% TODO: 补上写作思路
% 0. 一句话简单讲一下overview
% 1. 首先得到RGB image
% 2. 然后得到monocular depth
% 3. 然后根据monocular depth得到triangular mesh
% 4. 然后根据triangular mesh做warping
% 5. 最后用mesh renderer得到semantic maps at novel views
%
Our approach warps the given semantic map to novel views through the depth-based warping technique.
%
We first convert the input semantic map to the corresponding RGB image using SPADE~\cite{park2019semantic}, and then use monocular depth estimation networks~\cite{ranftl2020towards} to predict the depth map from the generated RGB image.
%
Then, a 3D triangular mesh is constructed based on the predicted depth following Shih \etal \cite{Shih20203DPU}.
%
The semantic mask is lifted to the mesh, whose vertices' color is assigned as the corresponding semantic label.
% After obtaining depth map, we lift the semantic mask into a 3D triangular mesh by treating each pixel as vertices and connecting them with their neighbors.
%
The 3D triangular mesh generated in such a manner may contain spurious edges due to the depth discontinuities in the depth map.
%
To solve this problem, we thus remove such edges according to the gradient of the depth map\yl{a bit more specific? I can guess the meaning but not very clear}. 
%
Eventually, we warp the semantic label map to the novel views using a mesh renderer following \tocite
%
%Finally, we warp the semantic label map to the novel views using a mesh renderer.

\paragraph{Semantic Inpainting}\label{sr}
%
Directly warping the given semantic map to novel views brings many holes in disocclusion regions.
%
To generate the missing contents, we train an inpainting network on single-view image collections using the self-supervised technique in \cite{han2022single}.
%
Specifically, we first use a pre-trained image segmentation model and a monocular depth estimation model to produce semantic maps and depth maps for the RGB images.
%
We then use the depth map $\mathbf{D}_i$ at source view $i$ to warp the original semantic mask $\mathbf{S}_i$ to a random target view $j$, obtaining warped semantic mask $\mathbf{S'}_j$ and depth map $\mathbf{D'}_j$ at target view $j$\yl{use $\bD$ and $\bS$ for consistency?}. 
%After directly warping the given semantic map to novel views, there exist many invisible areas at novel views. To overcome this problem, we train an inpainting network to fill in contents of semantic maps at these invisible regions. The semantic inpainting network is trained on the LHQ dataset~\cite{skorokhodov2021aligning}. We adopt a warp-back training strategy similar to~\cite{han2022single} to train our semantic inpainting network. Specifically, given the LHQ dataset, we use DeepLab-v2~\cite{chen2017deeplab} to produce semantic mask and use monocular depth estimation networks~\cite{ranftl2020towards} to predict the depth map for each image. Then, we use the depth map $D_i$ at source view $i$  to warp the original semantic mask $S_i$ to a random target view $j$, obtaining warped semantic mask $S_j'$ and depth map $D_j'$ at target view $j$. 
Next, We warp semantic mask $\mathbf{S'}_j$ back to the source view $i$ using depth map $\mathbf{D'}_j$, which generates a semantic mask $\mathbf{\hat{S}}_i$ with disocclusion region.
%
Finally, we input $\mathbf{\hat{S}}_i$ to the semantic inpainting network and train the networks to predict these disocclusion region with the ground truth semantic mask $\mathbf{S}_i$.
%
% After training, we warp the given semantic label map to each novel view and apply the inpainting network to fill in their invisible areas, thus obtaining multiview semantic label maps.
%
After training, we warp the given semantic mask $\mathbf{S}_0$ to each novel view to generate warped semantic masks $\mathbf{S'}_{1...N}$ and apply the semantic inpainting network to fill in their disocclusion region, thus obtaining multi-view semantic masks $\mathbf{S}_{1...N}$. 
%
% To infer the invisible contents at novel views, we train a semantic inpainting network on the Internet Dataset, LHQ~\cite{skorokhodov2021aligning}.
%
% 1. We adopt a warp-back training strategy similar to~\cite{han2022single}.
% 2. Specifically, given the LHQ dataset, 我们用DeepLab to produce segmentation maps and depth maps for each image.
% 3. Then, we use the depth map to warp the semantic map to a random target view $S_0'$, and then warp it back to the source view, which gives a semantic map with holes.
% 4. Finally, we input $\hat{S_0}$ to the inpainting network to predicted the complete semantic map.
% 5. The predicted semantic map is compared with the original semantic map to optimize the inpainting network.
% 6. After training, we warp the given semantic label map to each novel view and apply the inpainting network to fill in their invisible areas, thus obtaining multiview semantic label maps. 

% After directly warping the given semantic map to novel views, there exist many invisible areas at novel views.
% %
% To infer the invisible contents at novel views, we train a semantic refinement network on the Internet Dataset, LHQ.
% %
% In order to prepare the LHQ dataset to generate training data of our semantic refinement networks, we firstly use pretrained DeepLab-v2 to produce pseudo segmentation annotations and then use monocular depth estimation to predict the depth maps. We adopt a warp-back training strategy similar to Adampi.
% %
% In details, we warp the source semantic label map S0 to a random target view S0', and then warp it back to the source view to synthesize the semantic label map $\hat{S0}$ with naturalistic invisible areas.
% %
% Lastly, we input $\hat{0}$ to the semantic refinement networks and train the networks to fill in invisible areas. After training, we warp the given semantic label map to each novel view and apply semantic refinement network to fill in their invisible areas, thus obtaining multiview semantic label maps.

\paragraph{Semantic Field Fusion}
%
Although we obtain multi-view semantic masks aforementioned, we cannot directly use these semantic masks to guide the training of view synthesis. 
%
Because these multi-view semantic masks are not view consistent, directly using these semantic masks will cause artifacts. To tackle this problem, we introduce a semantic field to fuse multi-view semantic masks. Then, we use recovered semantic field to guide the training of view synthesis.

Here, we first give a brief introduction to the semantic field.
%
We adopt a continuous neural field to represent 3D semantic information and geometry, similar to~\cite{guo2022manhattan}.
%
We use a signed distance field $f_\theta$ to represent the geometry and add a semantic head $f_\phi$ to $f_\theta$ to learn the 3D semantic distribution $\mathbf{s}$. 
%
In details, $f_\theta$ maps a 3D coordinate $\mathbf{x}$ to an SDF value $\mathbf{\tilde{d}}$ \yl{better to use non-bold symbol as the $d$ is a scalar instead of a vector} and an intermediate feature $F_i$ of $c$ dimension, and the semantic head $f_\phi$ maps $F_i$ to semantic distribution $\mathbf{s}$:
% \vspace{-7 pt}
\begin{equation}\label{sn}
\begin{aligned}
&f_\theta: \mathrm{x} \in \mathbb{R}^3 \mapsto\left(\mathbf{\tilde{d}} \in \mathbb{R}, F_i \in \mathbb{R}^c\right) \\
&f_\phi: F_i \in \mathbb{R}^c \mapsto \mathrm{\mathbf{s}} \in \mathbb{R}^{M_s}
\end{aligned}
\end{equation}
where $M_s$ denotes the number of semantic classes. 
The expected semantic distribution $\mathbf{S}(\mathbf{r})$ and expected depth value $\mathbf{D}(\mathbf{r})$ of a camera ray $\mathbf{r}(t)=\mathbf{o}+t \mathbf{d}$ is obtained by volume rendering:
\begin{equation}
\begin{aligned}
\mathbf{S}(\mathbf{r})&=\sum_{i=1}^N T_i\left(1-\exp \left(-\sigma_i \delta_i\right)\right) \mathbf{s}_i\\
\mathbf{D}(\mathbf{r})&=\sum_{i=1}^N T_i\left(1-\exp \left(-\sigma_i \delta_i\right)\right) t_i\\
T_i&=\exp \left(-\sum_{j=1}^{i-1} \sigma_j \delta_j\right)
\end{aligned}
\end{equation}
where $\sigma_i$ is the density, which is induced by SDF value~\cite{yariv2021volume,wang2021neus}, and $\delta_k=t_{i+1}-t_i$ is the distance between adjacent points.


We apply the semantic loss \yl{to rendered 2D semantic masks} to learn the 3D semantic distribution:
\begin{equation}
\mathcal{L}_{\mathbf{S}}=-\sum_{\mathbf{r} \in \mathcal{R}} \sum_{k=1}^{M_s} \mathbf{S}_l^*(\mathbf{r}) \log \mathbf{S}_l(\mathbf{r})
\end{equation}
where $\mathbf{S}_l^*(\mathbf{r})$ is the ground truth semantic probability at class $l$, and $\mathbf{S}_l(\mathbf{r})$ is the rendered semantic probability at class $l$.

% 简单介绍$\mathbf{r}(t)=\mathbf{o}+t \mathbf{d}$
% 介绍sdf和semantic information
% 用数学式子表达清楚field
% 写rendering 公式
% 写loss
% TODO: 接下来写作的思路不清楚，不用先说问题，再说做法。如果不先把semantic neural field定义清楚，别人不知道我们在优化什么。直接讲怎么做的：
%
% 1. Semantic neural field的定义
% 2. 训练Semantic neural field的loss
% TODO: "how to overfit a semantic field on a single 2D semantic map"这句话有点问题, 因为我们已经有multi-view semantic maps了。


However, how to recover the geometry of the semantic field from semantic masks is a really challenging problem. 
%
% TODO: "can not" -> "cannot". 有这个问题的都要改掉
Neural field needs multi-view RGB images or depth maps to learning 3D geometry, but multi-view semantic masks cannot provide sufficient 3D supervision.
%
Inspired by previous methods~\cite{wang2022neuris,yu2022monosdf}, we use monocular depth maps to supervise the neural field.
%
In details, we firstly use depth map at the reference view obtained by~\ref{sw} to supervise neural field.
%
To better leverage the geometry information of this depth map, we also warp the depth map to novel views using the mesh renderer to train neural field\yl{why warping a depth map needs mesh renderer? You mean render depth maps at novel views using the neural renderer?}. Nevertheless, the depth values at invisible areas at the novel view is still unknown.
%
% TODO: 这里不用再讲之前的方法。直接说：To handle this problem, we adopt a simple but effective way to supervised the learned geometry at these areas.
To handle this problem, we adopt a simple but effective way to supervised the learned geometry at these areas.
% TODO: "unkown" -> unknown, 其他地方也要改一下
We consider the monocular depth map as a relative cue and constrain the rendered depth  $D$ at these unknown areas to match this relative cue.\yl{what do you mean by ``relative'' cue?}
%
% TODO: "firstly" -> first, 其他地方也要改一下
We first convert the semantic masks at novel views to RGB images via SPADE and then use monocular depth estimation networks~\cite{ranftl2020towards} to predict depth maps $\hat{D}$. 
\yl{It is a bit confusing here as there are many types of depth maps: 1) your rendered depth, 2) the depth maps you used in ``semantic inpainting'', 3) the depth maps you predict here.}
%
We enforce rendered depth map $D$ at novel view $i$ consistent with the predicted monocular depth map $\hat{D}$ at novel views $i$ by ranking loss~\cite{chen2016single, xian2020structure},
as shown in equation~\ref{rank}.
%
\begin{small}
\begin{equation}\label{rank}
\begin{aligned}
\mathcal{L}_{rank}= \begin{cases}\log \left(1+\exp \left(-\ell\left(p_0-p_1\right)\right)\right), & \ell \neq 0 \\ \left(p_0-p_1\right)^2, & \ell=0\end{cases}
\end{aligned}
\end{equation}
\end{small}where $j$, $k$  denote the locations of the randomly sampled pixels at novel view $i$. $p_0=D_{ij}$ and $p_1=D_{ij}$ is the rendered depth values at location $j$ and $k$.
$\ell$ is induced by the predicted monocular depth $D_i$ and a tolerance threshold $\tau$. 
$p_0^*=D_{ij}$, $p_1^*=D_{ik}$ \yl{$p_0^*=\hat{D}_{ij}$, $p_1^*=\hat{D}_{ik}$?} are the the predicted monocular depth values at location $j$ and $k$:
\begin{small}
\begin{equation}\label{ol}
    \ell= \begin{cases}+1, & p_0^* - p_1^*>=\tau \\ -1, & p_0^* - p_1^*<=\tau \\ 0, & \text { otherwise }\end{cases}.
\end{equation}
\end{small}
Besides, we also use scale- and shift-invariant loss~\cite{ranftl2020towards, yu2022monosdf}:
\begin{equation}
\mathcal{L}_{depth}=\sum_{\mathbf{r} \in \mathcal{R}}\|(w D(\mathbf{r})+q)-\hat{D}(\mathbf{r})\|^2
\end{equation}
where $w$ and $q$ are used to align the scale and shift of $D$ and $\hat{D}$, which can be solved with a least-squares criterion~\cite{ranftl2020towards,eigen2014depth}. The overall loss is described in the supplementary material.

%
\paragraph{Discussion} 
Our key idea is firstly construct a semantic neural field from a single semantic maps and then train a neural renderer guided by obtained semantic neural field. The advantages of producing multi-view consistent semantic masks instead of directly using inpainted semantic masks to guide the view synthsis is that we can provide a multi-view consistent semantic supervision for the training of view synthesis.

\subsection{View Synthesis Based on Semantic Field}

\yl{a short overview missing here?}

\paragraph{Neural Scene Appearance}\label{sgr}
%
% 1. 先overview
% 2. 再介绍具体步骤
% 

% TODO:
% 1. 先介绍neural scene appearance.
% 2. 然后介绍surface-guided rendering.
To represent the appearance of natural scenes, we follow EG3D~\cite{chan2022efficient} 
and use a tri-plane representation to represent our appearance field.
We query the color at each point by projecting it to each feature plane to aggregate the feature $F_a$. Then, we concatenate the feature vector $F_a$ and  map it to the RGB value by MLPs.

\paragraph{Surface-guided Rendering}\label{sgr}
We use the geometry recovered by semantic field to guide rendering.
%
We first extract the mesh from neural SDF field and use the mesh to guided ray sampling. 
%
Similar to~\cite{lin2021efficient, neff2021donerf},  we only sample one point on the surface for each ray. 
%
By using surface guided rendering instead of volume rendering, we can ensure view consistency. 
%
Additional advantage of adopting surface-guided rendering is that we can minimize the computational burden of producing full-resolution images, achieving efficient training and fast rendering. 

\paragraph{Semantics-guided Training}\label{sgt}
% 1. 先overview
% 2. 再介绍具体步骤
% 3. appearance field
We train our appearance field guided by semantic field with reconstruction and adversarial losses.
%
We first use our semantic field to render view-consistent semantic masks.
Then, we convert the semantic masks to pseudo-ground truth images using SPADE.
%
Pseudo-ground truth images are used to train the appearance field by using perceptual loss~\cite{johnson2016perceptual}:
\begin{equation}
\mathcal{L}_{\text {feat }}(\hat{C}, C)=\left\|\phi(\hat{C})-\phi(C)\right\|_2^2
\end{equation}
where $\hat{C}$ is the pseudo-ground truth image and $C$ is the rendered image. $\phi$ denotes VGG network~\cite{simonyan2014very}.
%
Perceptual loss makes training procedure more stable and faster.

Additionally, we use the adversarial loss to make the rendered images more photo-realistic.
%
We treat our rendered images as ‘fake’ samples,  pseudo-ground truth images as ‘real’ samples. We adopt OASIS discriminator~\cite{sushko2020you} as our discriminator, and use the same generator and discriminator loss as~\cite{sushko2020you}.

% TODO: 这里讨论相对于single-view view synthesis方法的优势
\paragraph{Discussion} 
The advantage of our semantic-guided training procedure is that we can fully exploit powerful generation capacity of SPADE at multiple viewpoint. Fusing multi-view information is much easier than directly predicting a 3D representation from a single view semantic mask.
% %
% Therefore, pseudo ground-truths generated by SPADE only differ in local texture, which is much easier for the appearance field to learn. 
% In addition, the supervision from the discriminator, which is conditioned on semantic maps, is consistent.

% \paragraph{Style Controlling}
% To make the style of our rendered images controllable, our triplane-based generator and pseudo-ground truth images are conditioned on the style code $z$. 
% During the training,  We periodically sample style code $z$ from a Gaussian distribution $N(0, 1)$ to encourage the generator to learn different styles.

